Generalized hybrid iterative methods for large-scale Bayesian inverse problems

We develop a generalized hybrid iterative approach for computing solutions to large-scale Bayesian inverse problems. We consider a hybrid algorithm based on the generalized Golub-Kahan bidiagonalization for computing Tikhonov regularized solutions to problems where explicit computation of the square root and inverse of the covariance kernel for the prior covariance matrix is not feasible. This is useful for large-scale problems where covariance kernels are defined on irregular grids or are only available via matrix-vector multiplication, e.g., those from the Mat\'{e}rn class. We show that iterates are equivalent to LSQR iterates applied to a directly regularized Tikhonov problem, after a transformation of variables, and we provide connections to a generalized singular value decomposition filtered solution. Our approach shares many benefits of standard hybrid methods such as avoiding semi-convergence and automatically estimating the regularization parameter. Numerical examples from image processing demonstrate the effectiveness of the described approaches.

==> macro_list.tex <==
% general header (fold)
\RequirePackage{amsfonts}
\RequirePackage{amsmath}
\RequirePackage{alltt, moreverb}
\RequirePackage{showkeys, showidx}
\RequirePackage{graphicx}
\RequirePackage[utf8]{inputenc}
\RequirePackage{algorithm, algorithmic} 
\renewcommand{\algorithmiccomment}[1]{{(\sf #1)}}
\RequirePackage{color, colortbl}
\RequirePackage{rotating}
\RequirePackage{boxedminipage}
\RequirePackage{upgreek}
\RequirePackage{subfigure}
\usepackage{textcomp}


% special header (fold)
\newcommand{\widebar}{\bar}
\newcommand{\widecheck}{\check}

\newcommand{\fro} {\rm F}                                  % define Frobenius norm
\newcommand{\eps} {\varepsilon}                            % redefine epsilon
\newcommand{\D}   {{\rm D}}                                % differential D
\newcommand{\tol} {{\rm tol}}                              % tolerance
\newcommand{\e}   {\textnormal{e}}                         % Eulerian number
\newcommand{\clos}{\textnormal{Closure}}                   % closure
\newcommand{\im}  {\textnormal{Im }}                       % imaginary part
\newcommand{\re}  {\textnormal{Re }}                       % real part
\newcommand{\hf}  {\frac{1}{2}}                            % 1/2
\DeclareMathOperator*{\argmin}{arg\,min}                   % arg min
\renewcommand{\i} {\textnormal{i}}                         % imaginary unity
\renewcommand{\t} {^{\top}}                                % transpose, e.g. $A\t$
\renewcommand{\d} {{\rm d}}                                % differential d
\renewcommand{\H} {^{{\rm H}}}                             % Hermitian
% \newcommand{\norm} [2][]{\left\|#2\right\|_{#1}}           % f.e. \norm[\infty]{A-B}
\newcommand{\abs}  [2][]{\left|#2\right|_{#1}}             % f.e. \abs[\infty]{A-B}
\newcommand{\cond} [2][]{{\rm cond}_{#1}\left( #2 \right)} % f.e. \cond[\infty]{A}
\newcommand{\pow}  [1]  {^{\left(#1\right)}}               % brackets exponent
\newcommand{\sign} [1]  {{\rm sign\!}\left( #1 \right)}    % signum
\newcommand{\spann}[1]  {{\rm span\!}\left( #1 \right)}    % span of a function
% \renewcommand{\diag} [1]  {{\rm diag\!}\left( #1 \right)}    % diagonal of a matrix
\renewcommand{\ker}[1]  {{\rm ker\!}\left( #1 \right)}     % kernel of a function
\renewcommand{\vec}[1]  {{\rm vec}\left( #1 \right)}     % kernel of a function
\newcommand{\rank}[1]  {{\rm rank}\left( #1 \right)}     % kernel of a function
\newcommand{\ul}   [1]  {\underline{#1}}                   % shorted underline
% \newcommand{\trace}{\mathsf{trace}}
% \newcommand{\email}[1]  {\texttt{#1}}                      % email
\newcommand{\kron}{\otimes}                                % kronecker product
\newcommand{\acknowledgement}[1]{\noindent\textbf{Acknowledgement: }#1}   % acknowledgement

\newcommand{\bmx}{\left[ \begin{array}}
\newcommand{\emx}{\end{array} \right]}


% ---------------------------------------------------------------------------
% bold greek and latin characters and bold numbers (requires amsmath) (fold)

\newcommand{\bfGamma}{{\boldsymbol{\Gamma}}}
\newcommand{\bfDelta}{{\boldsymbol{\Delta}}}
\newcommand{\bfTheta}{{\boldsymbol{\Theta}}}
\newcommand{\bfLambda}{{\boldsymbol{\Lambda}}}
\newcommand{\bfXi}{{\boldsymbol{\Xi}}}
\newcommand{\bfPi}{{\boldsymbol{\Pi}}}
\newcommand{\bfSigma}{{\boldsymbol{\Sigma}}}
\newcommand{\bfUpsilon}{{\boldsymbol{\Upsilon}}}
\newcommand{\bfPhi}{{\boldsymbol{\Phi}}}
\newcommand{\bfPsi}{{\boldsymbol{\Psi}}}
\newcommand{\bfOmega}{{\boldsymbol{\Omega}}}
\newcommand{\bfalpha}{{\boldsymbol{\alpha}}}
\newcommand{\bfbeta}{{\boldsymbol{\beta}}}
\newcommand{\bfgamma}{{\boldsymbol{\gamma}}}
\newcommand{\bfdelta}{{\boldsymbol{\delta}}}
\newcommand{\bfepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\bfvarepsilon}{{\boldsymbol{\varepsilon}}}
\newcommand{\bfzeta}{{\boldsymbol{\zeta}}}
\newcommand{\bfeta}{{\boldsymbol{\eta}}}
\newcommand{\bftheta}{{\boldsymbol{\theta}}}
\newcommand{\bfvartheta}{{\boldsymbol{\theta}}}
\newcommand{\bfiota}{{\boldsymbol{\iota}}}
\newcommand{\bfkappa}{{\boldsymbol{\kappa}}}
\newcommand{\bflambda}{{\boldsymbol{\lambda}}}
\newcommand{\bfmu}{{\boldsymbol{\mu}}}
\newcommand{\bfnu}{{\boldsymbol{\nu}}}
\newcommand{\bfxi}{{\boldsymbol{\xi}}}
\newcommand{\bfo}{{\boldsymbol{o}}}
\newcommand{\bfpi}{{\boldsymbol{\pi}}}
\newcommand{\bfvarpi}{{\boldsymbol{\varpi}}}
\newcommand{\bfrho}{{\boldsymbol{\rho}}}
\newcommand{\bfvarrho}{{\boldsymbol{\varrho}}}
\newcommand{\bfsigma}{{\boldsymbol{\sigma}}}
\newcommand{\bfvarsigma}{{\boldsymbol{\varsigma}}}
\newcommand{\bftau}{{\boldsymbol{\tau}}}
\newcommand{\bfupsilon}{{\boldsymbol{\upsilon}}}
\newcommand{\bfphi}{{\boldsymbol{\phi}}}
\newcommand{\bfvarphi}{{\boldsymbol{\varphi}}}
\newcommand{\bfchi}{{\boldsymbol{\chi}}}
\newcommand{\bfpsi}{{\boldsymbol{\psi}}}
\newcommand{\bfomega}{{\boldsymbol{\omega}}}
\newcommand{\bfA}{{\bf A}}
\newcommand{\bfB}{{\bf B}}
\newcommand{\bfC}{{\bf C}}
\newcommand{\bfD}{{\bf D}}
\newcommand{\bfE}{{\bf E}}
\newcommand{\bfF}{{\bf F}}
\newcommand{\bfG}{{\bf G}}
\newcommand{\bfH}{{\bf H}}
\newcommand{\bfI}{{\bf I}}
\newcommand{\bfJ}{{\bf J}}
\newcommand{\bfK}{{\bf K}}
\newcommand{\bfL}{{\bf L}}
\newcommand{\bfM}{{\bf M}}
\newcommand{\bfN}{{\bf N}}
\newcommand{\bfO}{{\bf O}}
\newcommand{\bfP}{{\bf P}}
\newcommand{\bfQ}{{\bf Q}}
\newcommand{\bfR}{{\bf R}}
\newcommand{\bfS}{{\bf S}}
\newcommand{\bfT}{{\bf T}}
\newcommand{\bfU}{{\bf U}}
\newcommand{\bfV}{{\bf V}}
\newcommand{\bfW}{{\bf W}}
\newcommand{\bfX}{{\bf X}}
\newcommand{\bfY}{{\bf Y}}
\newcommand{\bfZ}{{\bf Z}}
\newcommand{\bfa}{{\bf a}}
\newcommand{\bfb}{{\bf b}}
\newcommand{\bfc}{{\bf c}}
\newcommand{\bfd}{{\bf d}}
\newcommand{\bfe}{{\bf e}}
\newcommand{\bff}{{\bf f}}
\newcommand{\bfg}{{\bf g}}
\newcommand{\bfh}{{\bf h}}
\newcommand{\bfi}{{\bf i}}
\newcommand{\bfj}{{\bf j}}
\newcommand{\bfk}{{\bf k}}
\newcommand{\bfl}{{\bf l}}
\newcommand{\bfm}{{\bf m}}
\newcommand{\bfn}{{\bf n}}
\newcommand{\bfp}{{\bf p}}
\newcommand{\bfq}{{\bf q}}
\newcommand{\bfr}{{\bf r}}
\newcommand{\bfs}{{\bf s}}
\newcommand{\bft}{{\bf t}}
\newcommand{\bfu}{{\bf u}}
\newcommand{\bfv}{{\bf v}}
\newcommand{\bfw}{{\bf w}}
\newcommand{\bfx}{{\bf x}}
\newcommand{\bfy}{{\bf y}}
\newcommand{\bfz}{{\bf z}}
\newcommand{\bfzero}{{\bf0}}
\newcommand{\bfone}{{\bf1}}
\newcommand{\bftwo}{{\bf2}}
\newcommand{\bfthree}{{\bf3}}
\newcommand{\bffour}{{\bf4}}
\newcommand{\bffive}{{\bf5}}
\newcommand{\bfsix}{{\bf6}}
\newcommand{\bfseven}{{\bf7}}
\newcommand{\bfeight}{{\bf8}}
\newcommand{\bfnine}{{\bf9}}


\newcommand{\mxA}{{\bf A}}
\newcommand{\mxB}{{\bf B}}
\newcommand{\mxC}{{\bf C}}
\newcommand{\mxD}{{\bf D}}
\newcommand{\mxE}{{\bf E}}
\newcommand{\mxF}{{\bf F}}
\newcommand{\mxG}{{\bf G}}
\newcommand{\mxH}{{\bf H}}
\newcommand{\mxI}{{\bf I}}
\newcommand{\mxJ}{{\bf J}}
\newcommand{\mxK}{{\bf K}}
\newcommand{\mxL}{{\bf L}}
\newcommand{\mxM}{{\bf M}}
\newcommand{\mxN}{{\bf N}}
\newcommand{\mxO}{{\bf O}}
\newcommand{\mxP}{{\bf P}}
\newcommand{\mxQ}{{\bf Q}}
\newcommand{\mxR}{{\bf R}}
\newcommand{\mxS}{{\bf S}}
\newcommand{\mxT}{{\bf T}}
\newcommand{\mxU}{{\bf U}}
\newcommand{\mxV}{{\bf V}}
\newcommand{\mxW}{{\bf W}}
\newcommand{\mxX}{{\bf X}}
\newcommand{\mxY}{{\bf Y}}
\newcommand{\mxZ}{{\bf Z}}
\newcommand{\mxSigma}{{\bf \Sigma}}

% (end)

% ---------------------------------------------------------------------------
% caligraphic characters (fold)

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}
% (end)

% ---------------------------------------------------------------------------
% blackboard characters (requires amsfont) (fold)

\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

\newcommand{\sfE}{{\sf E}}


\newcommand{\true}{\mathrm{true}}
\newcommand{\filter}{\mathrm{filter}}
\newcommand{\tsvd}{\mathrm{tsvd}}
\newcommand{\tik}{\mathrm{tik}}
\newcommand{\err}{\mathrm{err}}
\newcommand{\spl}{\mathrm{spl}}
\newcommand{\wie}{\mathrm{Wiener}}
\newcommand{\smooth}{\mathrm{smooth}}
\newcommand{\con}{\mathrm{con}}
\newcommand{\ssvd}{\mathrm{ssvd}}
\newcommand{\inv}{\mathrm{inv}}
\newcommand{\mse}{\mathrm{MSE}}
\newcommand{\ERR}{\mathrm{ERR}}


